Open Source Vizier: Distributed Infrastructure and API for Reliable and Flexible Blackbox Optimization

Vizier is the de-facto blackbox and hyperparameter optimization service across Google, having optimized some of Google's largest products and research efforts. To operate at the scale of tuning thousands of users' critical systems, Google Vizier solved key design challenges in providing multiple different features, while remaining fully fault-tolerant. In this paper, we introduce Open Source (OSS) Vizier, a standalone Python-based interface for blackbox optimization and research, based on the Google-internal Vizier infrastructure and framework. OSS Vizier provides an API capable of defining and solving a wide variety of optimization problems, including multi-metric, early stopping, transfer learning, and conditional search. Furthermore, it is designed to be a distributed system that assures reliability, and allows multiple parallel evaluations of the user's objective function. The flexible RPC-based infrastructure allows users to access OSS Vizier from binaries written in any language. OSS Vizier also provides a back-end ("Pythia") API that gives algorithm authors a way to interface new algorithms with the core OSS Vizier system. OSS Vizier is available at https://github.com/google/vizier.

==> _pythia.tex <==

% \chansoo{Let's leave the details of namespace allocations out of the paper. Algorithms dumping its state into json blob and algorithm asking for data are in fact a usual dataflow in other OSS packages, so don't need to oversell this.}
For moderately sized metadata, policies can write to Vizier database via PolicySupporter. 
for values of size of up to 10 MB.  For larger metadata, policies may store in the file system.
The namespace and key are strings and values can either be strings (e.g. json blobs) or byte encoding of a protobuf. 
larger objects can be named in the metadata and stored in a filesystem.
 Each algorithm gets a top-level namespace that it can write; a special namespace is writeable by Vizier's users who can use it to communicate with Pythia algorithms or for their own purposes.
Pythia policies are expected to operate statelessly if necessary. Specifically, if saved state is missing or it is no longer compatible with the latest version of the algorithm running in service, the algorithm should make best effort to reconstruct its state by reading \texttt{Study}'s \texttt{Trial}s, generate suggestions, and then save the new state. This is useful to allow for fault tolerance (Section~\ref{sec:infra}), for upgrades to algorithms in the midst of studies, and it also gives the Vizier system and its users the flexibility to switch from one algorithm to another.
Pythia policies are not passed \texttt{Trial}s; rather, the algorithm is passed a \texttt{PolicySupporter} instance, which is an client-like API that allows it to read \texttt{Trials} (with their associated metadata tables).  Subject to access controls, the \texttt{PolicySupporter} also allows algorithms to read \texttt{Trials} and \texttt{StudySpec}s from other studies. We anticipate that an algorithm might save enough state so that it only needs to read the Trials that have been completed since it last ran; this can be a major efficiency improvement over e.g. \citep{vizier_v1} for e.g. evolutionary algorithms for large studies.
We outline the intended usage in Code Block \ref{lst:pythia1}.

\begin{lstlisting}[label={lst:pythia1}, float=h, language=Python, frame=tlrb, captionpos=b, caption={Pseudocode for implementing a Pythia policy's main \texttt{suggest} and additional \texttt{early\_stop} implementations, with use of the \texttt{PolicySupporter} to selectively obtain old trial data. Use of ``\text{...}" means that it is to be replaced with user-dependent input.}]
from vizier.service.pythia2.base import Policy
from vizier.service.pythia_supporter import PolicySupporter

class MyPolicy(Policy):
  def __init__(self, policy_supporter: PolicySupporter):
    self.policy_supporter = policy_supporter  # Used to obtain old trials.

  def suggest(self, request: base.SuggestRequest) -> List[base.SuggestDecision]:
    """Suggests trials to be evaluated."""
    suggestions = []
    for _ in range(request.count):
      old_trials = self.policy_supporter.GetTrials(...)
      trial = make_new_trial(old_trials, request.study_config)
      suggestions.append(base.SuggestDecision(trial))
    return suggestions

  def early_stop(
      self, request: base.EarlyStopRequest) -> List[base.EarlyStopDecision]:
    """Selects trials to stop from the request."""
    old_trials = self.policy_supporter.GetTrials(...)
    trials_to_stop = determine_trials_to_stop(old_trials, request.trial_ids)
    return [base.EarlyStopDecision(id) for id in trials_to_stop]
\end{lstlisting}


\url{https://github.com/googleapis/python-aiplatform/blob/main/google/cloud/aiplatform_v1beta1/types/study.py}


==> outline.tex <==

\subsection{Paper Structure}

\begin{enumerate}
\item Intro
\item General concepts and object hierarchy (with tree visualization perphaps?): Study, StudyConfig, SearchSpace, MetricInformation, Trial, Measurement, Metric, etc.
\all{Decide where to explain conditional search and multi-metric search}
\item Pythia and PolicySupporter API
  \begin{enumerate}
      \item Stateless design: More details on Trial's pending state and how pythia is designed with service deployment in mind.
      \item Stateful algorithms can still be efficiently implemented by using metadata. Case study on RegEvo/Firefly/NSGA2.
   \end{enumerate}
\item keras and tfp modules
   \begin{enumerate}
      \item Overview of GP-UCB implementation explaining the key components.
      \item XLA compilation and speed
      \item Robustness
   \end{enumerate}
\item Raytune plugin \all{Do we want to make comparsions to Ax / BoTorch / Raytune?}
\item Benchmarks:
\begin{enumerate}
\item Compare among our implementations (e.g. random vs gp-ucb), not against the outside world.
\item (Reach) Compare reliability (e.g. exceptions due to uncaught cholesky failures) to one or two widely used OSS packages (e.g. HEBO, Raytune, BoTorch?).
\end{enumerate}
\end{enumerate}

==> storage.tex <==

\begin{table}[h]
\begin{center}
\begin{tabular}{ |c|c|c|c| } 
\hline
Name & What is it? & What does it contain? & Extra Information \\ 
\hline \hline
Study & All data relevant to optimization over $f(x)$ & StudySpec, List of Trials & \\
Trial & Single evaluation of $f(x)$ & Scalar value $f(x) \in \mathbb{R}$ and $x \in \mathcal{X}$ & \\ 
StudySpec & Specification of a study. & Multiple ParameterSpecs combined to form $\mathcal{X}$ & \\
ParameterSpec & Specification of a parameter & & \\
MetricSpec & & & \\

\hline
\end{tabular}
\end{center}
\caption{Organization of terms in Vizier. \textcolor{red}{Change to picture}}
\label{table:definitions}
\end{table}

==> tfp_and_keras.tex <==

\section{Default Algorithm Modules}
To provide users a set of pre-existing modules to assist in constructing a broad variety of algorithms, OSS Vizier also contains implemented classes from TensorFlow Probability and Keras.

\subsection{TensorFlow Probability}
\textcolor{red}{Talk about TFP, citations, how to deal with cholesky stability issues, why it makes a good software to write BayesOpt + other algorithms.  Need to highlight which parts are used in the default algorithm modules that have been open-sourced.}

\todo{BayesFlow+chansoo}

TensorFlow Probability (TFP) \citep{tfp} is a Python library for probabilistic modeling and statistical analysis using TensorFlow \citep{tf} or JAX [cite].  TFP enables practitioners to combine probabilistic models and deep learning, while taking advantage of automatic differentiation, as well as modern parallel and vectorized hardware -- multi-core CPUs, as well as Graphical Processing Units (GPUs) and Tensor Processing Units (TPUs) [cite TPU paper].

TFP offers many critical building blocks for implementing Bayesian optimization, which include:

\paragraph{Modeling Random Functions}  For modeling random functions, TFP provides implementations of Gaussian Process (GP) prior and posterior distributions, along with a library of popular positive-definite kernels (exponentiated quadratic, Matern, periodic, etc.) that can be combined to build covariance functions.  TFP also includes an extensive library of probability distributions for specifying prior distributions for model hyperparameters.

TODO: ARD and input warping.

TODO: Multi-task GPs and kernels.

In addition to GPs, TFP can be used to model unknown objective functions as Student-t Processes [cite Shah 2014?], Bayesian Structural Time Series models [cite?], and Bayesian Neural Networks.

\paragraph{Robust Cholesky Decomposition} TFP's Gaussian Process inference uses TensorFlow's batched Cholesky decomposition.  Due to limited numerical precision, we can encounter covariance matrices that are (or are nearly) indefinite and for which the Cholesky decomposition fails.  We use the standard technique \citep{diagonal_review,neal_1997} of adding a small constant ("jitter") to the diagonal of the covariance matrix to avoid such failures.  In particular, if the Cholesky decomposition fails for a covariance matrix, we retry several times, adding exponentially larger jitter each time.

TODO?: We could say something about improving this with an efficient, batched "modified Cholesky" in TF/JAX.


\paragraph{Inference}  TODO: MMAP inference via L-BFGS.  Full posterior inference via MCMC [cite tfp.mcmc paper?] or variational inference.  (Say something about reparmaeterization for gradient-based inference for MC acquisition functions?)  (Scalable variational GPs?)

Anything else to say about optimizing acquisition functions?


\subsection{Keras}

